MMA: A Momentum Mamba Architecture for Human Activity Recognition with Inertial Sensors

Human activity recognition (HAR) from inertial sensors is essential for ubiquitous computing, mobile health, and ambient intelligence. Conventional deep models such as Convolutional Neural Networks (CNNs), Recurrent Neural Networks (RNNs), and transformers have advanced HAR but remain limited by vanishing or exloding gradients, high computational cost, and difficulty in capturing long-range dependencies. Structured state-space models (SSMs) like Mamba address these challenges with linear complexity and effective temporal modeling, yet they are restricted to first-order dynamics without stable longterm memory mechanisms. We introduce Momentum Mamba, a momentum-augmented SSM that incorporates second-order dynamics to improve stability of information flow across time steps, robustness, and long-sequence modeling. Two extensions further expand its capacity: Complex Momentum Mamba for frequency-selective memory scaling. Experiments on multiple HAR benchmarks demonstrate consistent gains over vanilla Mamba and Transformer baselines in accuracy, robustness, and convergence speed. With only moderate increases in training cost, momentum-augmented SSMs offer a favorable accuracy-efficiency balance, establishing them as a scalable paradigm for HAR and a promising principal framework for broader sequence modeling applications.

==> content/_abstract.tex <==
\begin{abstract}
Human activity recognition (HAR) from inertial sensors is essential for ubiquitous computing, mobile health, and ambient intelligence. Conventional deep models such as Convolutional Neural Networks (CNNs), Recurrent Neural Networks (RNNs), and transformers have advanced HAR but remain limited by \un{vanishing or exloding gradients} \tmn{not sure gradient instability is the right technical word}, high computational cost, and difficulty in capturing long-range dependencies. Structured state-space models (SSMs) like Mamba address these challenges with linear complexity and effective temporal modeling, yet they are restricted to first-order dynamics without \un{stable long-term memory mechanisms} \tmn{not sure this is the right work or should we mention it here. In general, oscillatory is not good}. We introduce Momentum Mamba, a momentum-augmented SSM that incorporates second-order dynamics to \un{improve stability of information flow across time steps} \tmn{This will cause confusion, since they will think that we enhance the model's training}, robustness, and long-sequence modeling. Two extensions further expand its capacity: Complex Momentum Mamba for \un{frequency-selective} memory \tmn{jargon. What does it mean? It is better to use simple words} and Adam Momentum Mamba for adaptive \un{gradient} scaling \tmn{it is not adaptive momentum. It is adaptive gradient}. Experiments on multiple HAR benchmarks demonstrate consistent gains over vanilla Mamba and Transformer baselines in accuracy, robustness, and convergence speed. With only moderate increases in training cost, \un{momentum-augmented} SSMs \tmn{not consistent. You call it momentum-augmented SSM above} offer a favorable accuracy-efficiency trade-off, establishing them as a scalable paradigm \tmn{why scalable?} for HAR and a promising \un{principal framework} \tmn{I would not use the word foundation here. Maybe ``a principal framework''} for broader sequence modeling applications.
\end{abstract}

==> content/continuous_momentum.tex <==
\subsection{Preliminaries: Continuous-Time Structured State-Space Models (S4)}

State space models (SSMs) offer a principled approach to modeling temporal dependencies by encoding input sequences through latent dynamical systems. The S4 model, a structured variant of SSMs, formulates the transformation of a 1D input signal $x(t) \in \mathbb{R}$ into an output $y(t) \in \mathbb{R}$ through a continuous-time latent state $h(t) \in \mathbb{R}^N$, governed by the following equations.
\begin{align}
    h'(t) &= A h(t) + B x(t) \label{eq:s4-continuous-dynamics} \\
    y(t) &= C h(t) \label{eq:s4-continuous-output}
\end{align}
Here, $A \in \mathbb{R}^{N \times N}$ is the state transition matrix that governs the internal dynamics, and $B \in \mathbb{R}^{N \times 1}$ and $C \in \mathbb{R}^{1 \times N}$ are projection matrices that map the input to the state and the state to the output, respectively. 

The continuous formulation of S4 serves as a foundation for efficient and scalable sequence modeling, particularly in long-context scenarios.

\subsection{Heavy-Ball Momentum for Continuous-Time S4}

To overcome the expressive limitations of conventional first-order State-Space Models (SSMs), we propose a second-order formulation inspired by the Heavy-Ball momentum method \cite{polyak1964some}. Originally developed to accelerate convergence in convex optimization, this method introduces inertia and damping into the system, enabling the modeling of both transient oscillations and long-range dependencies.

The dynamics of the proposed system are governed by a second-order differential equation:
\begin{align}
    h''(t) + \gamma h'(t) &= -A h(t) + B x(t) + b
    \label{eq:heavyball_secondorder} \\
    y(t) &= C h(t) + D x(t) \label{eq:heavyball_output}
\end{align}
where $h(t) \in \mathbb{R}^N$ is the latent state, $x(t) \in \mathbb{R}^D$ the input, and $y(t) \in \mathbb{R}^M$ the output. The damping coefficient $\gamma > 0$ controls friction-like behavior, $A \in \mathbb{R}^{N \times N}$ (assumed diagonal) governs the internal dynamics, $B$, $C$, and $D$ are projection and feedthrough matrices, and $b$ is a learnable bias.

To express this system in canonical first-order form, we introduce an auxiliary velocity variable $z(t) = h'(t)$. Omitting the bias term $b$ and the direct readout from $x(t)$ for clarity, we obtain the following equivalent formulation:
\begin{align}
    z'(t) + \gamma z(t) &= -A h(t) + B x(t) \label{eq:heavyball_firstorder_z} \\
    h'(t) &= z(t) \label{eq:heavyball_firstorder_h}
\end{align}

\subsection{Discretizing the Heavy-Ball S4 Model}

To ensure numerical stability and computational efficiency, we discretize the continuous-time Heavy-Ball S4 system using an implicit integration scheme. Let $\Delta_n > 0$ denote the time step, and define discrete time indices $t_n = n \Delta_n$. Applying backward Euler discretization to the first-order system in Eqs.~\eqref{eq:heavyball_firstorder_z}–\eqref{eq:heavyball_firstorder_h} yields:
\begin{align}
    \frac{z_n - z_{n-1}}{\Delta_n} + \gamma z_n &= -A h_n + B x_n \label{eq:disc_z_1} \\
    \frac{h_n - h_{n-1}}{\Delta_n} &= z_n \label{eq:disc_h_1}
\end{align}

Multiplying by $\Delta_n$ and rearranging leads to the update equations:
\begin{align}
    (1 + \gamma \Delta_n) z_n + \Delta_n A h_n &= z_{n-1} + \Delta_n B x_n, \label{eq:disc_z_2} \\
    h_n &= h_{n-1} + \Delta_n z_n. \label{eq:disc_h_2}
\end{align}

We define the augmented state $s_n = \begin{bmatrix} z_n \\ h_n \end{bmatrix} \in \mathbb{R}^{2N}$, which allows the system to be written compactly as:
\begin{align}
    M s_n = s_{n-1} + F_n, \label{eq:disc_aug_system}
\end{align}
where:
\begin{align}
    M =
    \begin{bmatrix}
        1 + \gamma \Delta_n & \Delta_n A \\
        - \Delta_n I & I
    \end{bmatrix}, \quad
    F_n =
    \begin{bmatrix}
        \Delta_n B x_n \\
        0
    \end{bmatrix}. \label{eq:disc_matrices}
\end{align}

Since $A$ is diagonal, $M$ admits a closed-form inverse via the Schur complement:
\begin{align}
    M^{-1} =
    \begin{bmatrix}
        S & -\Delta_n A S \\
        -\Delta_n S & (1 + \gamma \Delta_n) S
    \end{bmatrix}, \label{eq:m_inverse}
\end{align}
where $S = \left(1 + \gamma \Delta_n + \Delta_n^2 A \right)^{-1}$ is a diagonal matrix and can be inverted element-wise. The recurrence becomes:
\begin{align}
    s_n = M^{-1} s_{n-1} + M^{-1} F_n. \label{eq:disc_recurrence}
\end{align}

\textbf{Stability and expressiveness.}
The implicit integration scheme guarantees global asymptotic stability, provided the eigenvalues of $M^{-1}$ are bounded. This is ensured if all diagonal entries of $A$ are non-negative. The damping term $\gamma$ dissipates energy over time, while the second-order dynamics allow the model to represent richer temporal patterns, including oscillations and long-range dependencies. Notably, the latent state dimension is effectively doubled from $N$ to $2N$.

\textbf{Fast recurrence via associative parallel scans.}
Beyond stability, the affine recurrence in Eq.~\eqref{eq:disc_recurrence} supports efficient parallel computation. Since $M$ is time-invariant, the update:
\begin{align}
    s_n = M s_{n-1} + F_n
\end{align}
can be interpreted as a scan over a sequence of affine transformations. This operation is associative under the binary operator:
\begin{align}
    (a_1, a_2) \bullet (b_1, b_2) = (b_1 a_1, b_1 a_2 + b_2),
\end{align}
which combines pairs of affine transformations into a single equivalent transformation.

This associativity enables the full sequence $\{s_n\}_{n=1}^L$ to be computed in $\mathcal{O}(\log L)$ time using a parallel prefix scan algorithm \cite{kogge1973parallel, blelloch1990prefix}. Specifically, applying a scan over the input sequence of affine pairs $\{(M, F_1), (M, F_2), \ldots, (M, F_L)\}$ yields intermediate states:
\begin{align}
    \left\{(M, F_1),\ (M^2, M F_1 + F_2),\ \ldots,\ (M^L, \sum_{i=1}^L M^{L-i} F_i) \right\},
\end{align}
where the solution to the recurrence with initial state $s_0 = 0$ is stored in the second component of each pair. 

This technique—referred to as an \textit{implicit parallel scan}—has proven effective in recent state-space models such as S5 and LinOSS \cite{smith2023simplified, rusch2024oscillatory}. Our model inherits these advantages, offering both expressive second-order dynamics and fast parallel inference suitable for modern accelerator hardware.

\subsection{Deriving the Heavy-Ball Formulation for Mamba (S6)}

We now extend the second-order dynamics of the Heavy-Ball S4 system to a discrete-time, input-conditioned formulation inspired by the Mamba (S6) architecture. While standard Mamba discretizes continuous-time state-space models using Zero-Order Hold (ZOH), in this work we adopt an alternative route based on implicit Euler discretization. This approach is both numerically stable and computationally efficient, and naturally accommodates the second-order latent dynamics introduced by Heavy-Ball momentum.

To begin, we consider the continuous-time second-order system:
\begin{align}
    h''(t) + \gamma h'(t) = -A(t) h(t) + B(t) x(t),
\end{align}
which can be rewritten in first-order form by defining the velocity state $z(t) = h'(t)$:
\begin{align}
    z'(t) + \gamma z(t) &= -A(t) h(t) + B(t) x(t), \\
    h'(t) &= z(t).
\end{align}

Applying backward Euler discretization with a (possibly input-dependent) step size $\Delta_n > 0$, we obtain:
\begin{align}
    \frac{z_n - z_{n-1}}{\Delta_n} + \gamma z_n &= -A_n h_n + B_n x_n, \\
    \frac{h_n - h_{n-1}}{\Delta_n} &= z_n,
\end{align}
which simplifies to the following recurrence:
\begin{align}
    (1 + \gamma \Delta_n) z_n + \Delta_n A_n h_n &= z_{n-1} + \Delta_n B_n x_n, \label{eq:euler_disc_z} \\
    h_n &= h_{n-1} + \Delta_n z_n. \label{eq:euler_disc_h}
\end{align}

Here, $A_n$, $B_n$, and $\Delta_n$ are input-conditioned matrices or scalars derived from learned transformations of $x_n$; $\gamma > 0$ is a learnable or fixed damping coefficient; $z_n \in \mathbb{R}^N$ is the auxiliary velocity state; and $h_n \in \mathbb{R}^N$ is the primary hidden state.

We now define the augmented latent state $s_n = \begin{bmatrix} z_n \\ h_n \end{bmatrix} \in \mathbb{R}^{2N}$, and represent the recurrence compactly as:
\begin{align}
    M_n s_n = s_{n-1} + F_n,
\end{align}
with:
\begin{align}
    M_n &=
    \begin{bmatrix}
        1 + \gamma \Delta_n & \Delta_n A_n \\
        - \Delta_n I & I
    \end{bmatrix}, \quad
    F_n =
    \begin{bmatrix}
        \Delta_n B_n x_n \\
        0
    \end{bmatrix}.
\end{align}

Assuming $A_n$ is diagonal (as in Mamba), the matrix $M_n$ is invertible and admits a closed-form inverse via the Schur complement:
\begin{align}
    M_n^{-1} =
    \begin{bmatrix}
        S_n & -\Delta_n A_n S_n \\
        -\Delta_n S_n & (1 + \gamma \Delta_n) S_n
    \end{bmatrix}, 
    \\
    \quad S_n = \left(1 + \gamma \Delta_n + \Delta_n^2 A_n\right)^{-1}.
\end{align}
This yields the final recurrence:
\begin{align}
    s_n = M_n^{-1} s_{n-1} + M_n^{-1} F_n,
\end{align}
from which we recover $h_n$ by selecting the second block of $s_n$. The output is then computed as:
\begin{align}
    y_n = \boldsymbol{C}_n h_n,
\end{align}
where $\boldsymbol{C}_n$ is either a fixed or input-conditioned projection matrix.

This formulation generalizes Mamba to a second-order latent dynamical system by incorporating velocity states and damping into the recurrence. Unlike ZOH-based discretization, Euler-based integration allows explicit control over numerical stiffness and smoother handling of high-frequency input variations. We refer to this architecture as \textbf{Heavy-Ball Mamba}, as it embeds momentum-like behavior into the hidden state evolution.

The model retains the key inductive biases of Mamba—selective recurrence, efficient parallelization via associative scans, and content-aware computation—while enriching its temporal modeling capacity with oscillatory and inertial dynamics. This extension enables the model to represent richer temporal patterns and improves learning stability for long-range sequence modeling.

==> content/har_system_.tex <==
% \begin{figure}%[htbp]
%     \flushleft
%     \includegraphics[width=0.9\columnwidth]{Images/architecture.png}
%     \caption{Overall architecture of the proposed MMA system. Six-axis inertial signals are processed by convolutional and normalization layers, followed by stacked Momentum Mamba blocks that capture both short- and long-range dependencies. The aggregated representation is mapped to activity classes through a global pooling and linear classifier.}
%     \label{fig:HAR_arch}
% \end{figure}

\un{The overall architecture of the proposed \textit{Momentum Mamba} framework for inertial HAR is illustrated in Fig.~\ref{fig:momentum_mamba_arch}. The framework is designed to efficiently process synchronized six-axis inertial measurement unit (IMU) signals and to predict per-window activity labels through three main components: (\textit{i}) a convolutional front-end, (\textit{ii}) a momentum-augmented Mamba backbone, and (\textit{iii}) a lightweight classification head.}

\subsection{Convolutional Front-End}
\un{The first stage of the MMA employs a lightweight one-dimensional convolutional encoder that transforms raw six-axis inertial measurements (accelerometer and gyroscope) into high-dimensional temporal feature maps. A 1D convolutional layer with kernel size $3$ captures local temporal dependencies within short motion windows, followed by batch normalization, ReLU activation, and dropout for regularization. This design enhances local feature extraction and mitigates sensor noise, effectively projecting raw low-dimensional signals into a richer feature space for subsequent state-space processing.}

\un{The front-end is intentionally lightweight (about $1.8$K parameters for $6\!\rightarrow\!256$ dimensions), ensuring computational efficiency suitable for edge deployment. Its core purposes are threefold: (\textit{i}) capture local temporal patterns characteristic of human motion dynamics such as acceleration-deceleration transitions, (\textit{ii}) expand the representational capacity of sensor streams before entering the Momentum Mamba backbone, and (\textit{iii}) provide initial noise filtering through learned convolutions. Consequently, this module reduces the effective sequence length while enriching feature diversity, serving as an efficient bridge between raw IMU inputs and the momentum-augmented state-space layers that model long-range temporal dependencies in human activity recognition.}

\subsection{Momentum Mamba Backbone}
\un{The proposed framework extends the standard Mamba (S6) backbone by integrating a momentum mechanism inspired by second-order optimization dynamics. This modification, detailed in Section~IV of the Momentum Mamba formulation, introduces an auxiliary velocity state alongside the hidden state, forming a dual-state recurrence that enhances long-range temporal modeling and stabilizes gradient propagation.}

\un{The momentum-augmented update incorporates a smoothed velocity term that accumulates temporal information over time. This design reshapes the Jacobian spectrum, mitigating exponential gradient decay and improving robustness against high-frequency sensor noise--all while preserving the linear-time complexity of SSMs. As a result, MMA achieves smoother hidden-state evolution, stronger resilience to transient perturbations, and more stable convergence across long sequences.}

\un{The momentum mechanism provides a physically grounded inductive bias well suited for inertial signals: 
\begin{itemize}
\item \textbf{Inertial consistency:} The auxiliary velocity state captures the gradual, inertia-driven nature of human motion. 
\item \textbf{Noise robustness:} Temporal smoothing through momentum decay filters sensor noise while preserving activity-level dynamics. 
\item \textbf{Smooth transitions:} The model naturally represents gradual activity changes (e.g., walking $\rightarrow$ standing). 
\item \textbf{Extended dependencies:} The accumulated momentum state enables effective modeling of long-duration activities. 
\end{itemize}}

\un{Despite the additional momentum pathway, MMA retains linear-time complexity in sequence length $L$. Parallel scan (prefix-sum) implementations allow efficient computation of both $\mathbf{v}_t$ and $\mathbf{h}_t$, preserving GPU-friendly execution. Compared to vanilla Mamba, the overhead in training time and VRAM usage is marginal ($<5\%$ increase).}

\subsection{Classification Head}
\un{The final stage of the architecture aggregates the temporal representations obtained from the Momentum Mamba backbone into compact embeddings for activity classification. As formulated in Section IV, the hidden representations $\mathbf{h}_t$ produced at each time step are averaged along the temporal dimension to form a global feature descriptor, which is subsequently projected through a fully connected linear layer to produce class logits for $C$ activity categories.}

\un{This simple yet effective design introduces minimal additional parameters (less than 0.5\% of the total), ensuring a favorable trade-off between accuracy and efficiency. The use of global average pooling provides a holistic summary of temporal dynamics, while the linear projection enables direct mapping from latent representations to activity labels.}

\subsection{Summary}
\un{In summary, the proposed \textit{Momentum Mamba} framework establishes a principled and efficient approach to inertial human activity recognition by combining lightweight convolutional encoding, momentum-augmented state-space modeling, and compact classification. The integration of a momentum mechanism within the Mamba backbone provides several key advantages for HAR: it captures both transient and sustained motion patterns, preserves temporal continuity inherent in human movements, and stabilizes gradient propagation over long sequences. These properties enable the model to robustly distinguish activities that share overlapping short-term dynamics (e.g., walking vs.\ jogging) and to recognize complex behaviors that unfold over extended durations (e.g., cooking, exercising).}

\un{Furthermore, by maintaining linear-time complexity and a compact parameter footprint, MMA is well suited for deployment on wearable and mobile devices where computation and memory are constrained. The convolutional front-end effectively filters sensor noise and emphasizes local temporal structure, while the dual-state momentum backbone enriches temporal context through smooth, inertia-aware state transitions. Together, these components yield a model that is both physiologically interpretable and computationally efficient, advancing the robustness, accuracy, and real-time applicability of IMU-based human activity recognition systems.}


==> content/intro_.tex <==
Human activity recognition (HAR) aims to identify human actions from sensor data automatically and supports applications in healthcare~\cite{Sigcha2023DeepLA, Nemati2021CoughBuddyMC, Gao2019TowardsRA, Bhattacharya2022EnsemHARAE}, human-computer interaction~\cite{Zhang2018FingerPingRF, Phinyomark2018EMGPR}, lifestyle monitoring~\cite{Jha2023AHA,Wang2019AttentionBasedCN}, sports analysis, and ambient assisted living~\cite{Sigcha2023DeepLA, Karim2024HumanAR}. Traditional HAR systems have relied on visual inputs such as RGB videos, depth maps, and skeletal data~\cite{Sun2020HumanAR, pham2021combining, Ghosh2022DeepLM}, but these approaches face challenges of occlusion, lighting sensitivity, computational cost, and privacy concerns~\cite{Sun2020HumanAR, Yang2024PrivacypreservingHA}.  

These limitations have driven a growing transition toward non-visual modalities, particularly inertial sensing through accelerometers and gyroscopes \cite{Lima2019Human}. Due to the mass adoption of smartphones and wearable devices, IMU data have become increasingly ubiquitous and accessible for HAR applications~\cite{Zhang2021DeepLI}. Inertial HAR offers unique advantages: privacy preservation, low power consumption, and fine-grained motion capture suitable for continuous and real-time monitoring ~\cite{Ignatov2018RealtimeHA, Qi2020ASA}. However, modeling inertial data introduces its own challenges. Sensor signals are inherently noisy, lack spatial context, and require robust temporal modeling of multivariate time series under resource-constrained conditions~\cite{Ahad2021, chen2021deeplearningsensorbasedhuman}.

Deep learning has become the dominant paradigm for inertial HAR. Convolutional Neural Networks (CNN) extract local temporal patterns~\cite{zeng2014convolutional}, \un{whereas Recurrent Neural Networks (RNN) are designed to model sequential dependencies but often struggle to capture long-range temporal relationships due to issues such as vanishing gradients} ~\cite{Farid2025ASA, Bengio1994LearningLD} \tmn{does this conflict with what we write in the abstract: ``...RNNs ... difficulty in capturing long-range dependencies.''}. Hybrid CNN–RNN architectures have been developed to integrate the complementary strengths of both models~\cite{ordonez2016deep}. Transformer-based models~\cite{vaswani2017attention} \un{have been introduced to capture global contextual dependencies through self-attention mechanisms,} \tmn{not sure why global self-attention is a good thing. Maybe "capture the global context"} with HAR-specific extensions such as GAFormer~\cite{10317315} and MAMC~\cite{10705364}, but their quadratic \tmn{computational and memory} \un{computational and memory complexity causes the difficulty for real-time deployment} \tmn{how about: real-time deployment?}.  

Structured state-space models (SSMs) offer a scalable alternative \un{to Transformers, achieving linear-time complexity in sequence length. Among these, Mamba \cite{dao2024hungry} represents a significant advance, introducing an input-dependent selective mechanism that allows the model to dynamically focus on relevant information, with variants like HARMamba \cite{li2024harmamba} being adapted for HAR. Despite its effectiveness, Mamba's reliance on first-order dynamics can limit its ability to maintain stable gradient flow over long sequences, a critical challenge for noisy inertial data. The principle of incorporating second-order dynamics, inspired by momentum optimization methods \cite{polyak1964heavyball, Nesterov1983AMF, Sutskever2013OnTI} \tmn{2 more citations here}, offers a robust solution to this stability issue. This has been demonstrated in architectures such as MomentumRNN \cite{momentumRNN} and, more recently in the SSM context, by LinOSS \cite{rusch2025oscillatorystatespacemodels}, , which uses oscillatory dynamics for stable \un{long-range} \tmn{long-range} modeling. However, LinOSS employs time-invariant (i.e., static) state transition parameters that do not adapt to the input, thereby lacking the content-aware selectivity that is Mamba's key advantage. This exposes a clear research gap: no existing model integrates the adaptive selectivity of Mamba with the enhanced stability of second-order dynamics.} \tmn{what is static structures? Need to elaborate more}.\tmn{Also, it is not clear the disadvantage of structured SSMs?} \tmn{not sure recursions is the right word here. It should be second-order dynamics. Then, it is not clear why we are different from LinOSS. Maybe discussing about Momentum first, then mention LinOSS, and explain in detail why we are different from LinOSS}. 

\tmn{\bf Contribution:} We propose \textit{Momentum Mamba \un{(MMA)} \tmn{(MMA)}} architecture \tsout{(MMA)}, \tmn{a novel family of Mamba models} that augments Mamba’s \un{dynamics} \tmn{recurrence in SSM is also input-dependent. Just say: ``Mamba's dynamics''} with heavy-ball momentum. This integration enhances gradient stability, noise robustness, and temporal expressiveness while retaining linear scalability. Our contribution is three-fold:

\begin{enumerate}
    \item \un{We introduce \emph{Momentum Mamba}, the first selective state-space model (SSM) that integrates momentum-driven second-order dynamics for improving gradient stability and temporal modeling in long-sequence inertial HAR.} \tmn{We introduce \emph{Momentum Mamba}, the first selective state-space model (SSM) that integrates momentum-driven second-order dynamics for improving gradient stability and temporal modeling in long-sequence inertial HAR.}

    \item \un{We theoretically prove that Momentum Mamba achieves better-structured spectrum than the Mamba baseline Mamba, explaining to the model’s stability enhancement.} \tmn{experiments to verify the proposed method do not count as contributions. We should mention the theoretical contribution here and move it up as a second contribution. For example, ``We theoretically prove that Momentum Mamba achieves better-structured spectrum than the Mamba baseline Mamba, explaining to the model’s stability enhancement.''}

     \item \un{We demonstrate that the design principles of Momentum Mamba extend naturally to other advanced momentum-based optimization methods. In particular, we introduce Complex Momentum Mamba and Adam Momentum Mamba, which achieve frequency-selective memory via complex-valued momentum and adaptive control of momentum scaling, respectively.} \tmn{We demonstrate that the design principles of Momentum Mamba extend naturally to other advanced momentum-based optimization methods. In particular, we introduce Complex Momentum Mamba and Adam Momentum Mamba, which achieve frequency-selective memory via complex-valued momentum and adaptive control of momentum scaling, respectively.}.
\end{enumerate}

Extensive evaluations on \un{a variety of} \tsout{multiple} \tmn{a variety of} \tsout{publicly available} inertial HAR benchmarks demonstrate that our models consistently outperform transformer, vanilla Mamba, and oscillatory SSM baselines, achieving superior trade-offs in accuracy, convergence speed, and resource efficiency.

% Human activity recognition (HAR) is a rapidly evolving research field that focuses on automatically identifying human actions based on sensor data. It has gained significant attention due to its broad applicability in various domains, including healthcare (disease monitoring, rehabilitation, and elderly care)~\cite{Sigcha2023DeepLA, Nemati2021CoughBuddyMC, Gao2019TowardsRA, Bhattacharya2022EnsemHARAE}, human-computer interaction (gesture-based control and immersive AR/VR)~\cite{Zhang2018FingerPingRF, Phinyomark2018EMGPR}, fitness and lifestyle monitoring~\cite{Jha2023AHA, Wang2019AttentionBasedCN}, as well as sports performance analysis, surveillance, and ambient assisted living~\cite{Wang2019MotionRF, Karim2024HumanAR}. Traditional HAR systems are mainly based on visual modalities such as RGB videos, depth maps, and skeletal data~\cite{Sun2020HumanAR, pham2021combining, Ghosh2022DeepLM}. Although these modalities offer rich spatial and contextual information, they also pose several challenges, including sensitivity to lighting conditions, occlusions, high computational requirements, and significant concerns regarding user privacy.~\cite{Yang2024PrivacypreservingHA, Sun2020HumanAR}.

% These limitations have driven a growing transition toward nonvisual modalities, particularly inertial sensing through accelerometers and gyroscopes. Due to the mass adoption of smartphones and wearable devices, IMU data have become increasingly ubiquitous and accessible for HAR applications~\cite{Zhang2021DeepLI}. Inertial HAR offers unique advantages: privacy preservation, low power consumption, and fine-grained motion capture suitable for continuous and real-time monitoring ~\cite{Ignatov2018RealtimeHA, Qi2020ASA}. However, modeling inertial data introduces its own challenges. Sensor signals are inherently noisy, lack spatial context, and require robust temporal modeling of multivariate time series under resource-constrained conditions~\cite{Ahad2021, chen2021deeplearningsensorbasedhuman}.

% To address these challenges, deep learning has become the dominant paradigm in inertial HAR. Convolutional neural networks (CNNs) effectively extract local temporal patterns, while recurrent networks (RNNs), such as LSTMs and GRUs, capture sequential dependencies~\cite{ordonez2016deep, hammerla2016deep}. Despite their success, CNNs are limited by short receptive fields, and RNNs often suffer from vanishing gradients and high computational overhead. Transformer-based models~\cite{vaswani2017attention} introduced global self-attention, significantly advancing temporal modeling capacity. However, the quadratic complexity of attention remains a bottleneck for long sequences, hindering deployment in latency-critical or embedded scenarios.

% In parallel, momentum-inspired principles have proven powerful in both optimization and neural dynamics. Classical heavy-ball momentum~\cite{polyak1964heavyball} accelerates convergence and smooths gradient trajectories, while recent neural architectures demonstrate that second-order recursions improve gradient flow and long-horizon expressiveness. A related but distinct approach is the Linear Oscillatory State-Space Model (LinOSS)~\cite{rusch2025oscillatorystatespacemodels}, which augments selective SSMs with fixed oscillatory dynamics to guarantee universal approximation and stability. However, LinOSS operates within a static oscillatory framework and does not exploit momentum-based updates. This leaves an open gap between efficient selective SSMs and momentum-inspired mechanisms that can enhance robustness in noisy sensor environments.

% To bridge this gap, we propose a \textit{Momentum Mamba} architecture (MMA), the first integration of heavy-ball momentum into selective state-space recurrence. MMA enriches input-dependent dynamics with second-order updates, enhancing gradient stability, noise resilience, and temporal expressiveness while retaining the linear scalability of SSMs. Beyond the base model, we introduce Complex Momentum Mamba (frequency-sensitive memory) and Adam Momentum Mamba (adaptive momentum scaling), further broadening the flexibility of momentum-augmented SSMs for real-world deployment.

% Our key contributions are as follows:
% \begin{itemize}
%     \item \textbf{Momentum-augmented recurrence:} We propose \emph{Momentum Mamba}, which integrates heavy-ball momentum into Mamba’s input-dependent dynamics, improving robustness and stability in noisy inertial HAR streams.
    
%     \item \textbf{Extended architectures:} We design \emph{Complex Momentum Mamba} and \emph{Adam Momentum Mamba} to capture frequency-sensitive dynamics and enable adaptive momentum scaling, further enhancing the expressiveness and stability of momentum-driven SSMs.
    
%     \item \textbf{Comprehensive evaluation:} We benchmark Momentum Mamba and its variants on multiple inertial HAR datasets, consistently surpassing Mamba, Transformer, and oscillatory SSM baselines in accuracy and convergence.
% \end{itemize}

% The remainder of this paper is organized as follows. Section~\ref{sec:related_work} reviews related work, beginning with deep learning methods for inertial HAR, followed by structured state-space models with an emphasis on Mamba, and finally momentum-inspired approaches in neural dynamics. Section~\ref{sec:momentum_mamba} introduces the proposed Momentum Mamba method, detailing the integration of heavy-ball momentum into the Mamba architecture, the mitigation of vanishing gradients, and potential extensions using complex-valued and adaptive momentum mechanisms. Experimental evaluations are presented in Section~\ref{sec:experiments}, where we describe the benchmark datasets, implementation details, and performance comparisons. Finally, Section~\ref{sec:conclusion} concludes the paper and outlines future research directions.


==> content/prelim_.tex <==
 The classical state space model describes a continuous-time system that maps an input 
$x(t) \in \mathbb{R}$ to an output $y(t) \in \mathbb{R}$ via a hidden state 
$\mathbf{h}(t) \in \mathbb{R}^{d \times 1}$, formulated as:
\begin{equation}
\label{eqn:cssm}
\begin{aligned}
    \vh'(t) &= \mA\vh(t) + \mB x(t), \\
    y(t) &= \mC\vh(t) + D x(t),
\end{aligned}
\end{equation}
where $\mA \in \sR^{d \times d}$, $\mB,\vh(t), \vh'(t) \in \sR^{d \times 1}$, $\mC \in \sR^{1 \times d}$, and $D \in \sR$. The \emph{structured state space sequence models (S4)} are inspired by the classical SSMs and take the following discrete form of the continuous system in Eqn.~\ref{eqn:cssm}.
\begin{subequations}
    \begin{align}
        \vh_n &= \overline{\mA}\vh_{n-1} + \overline{\mB}x_n, \label{eqn:s4a} \\
        y_n &= \mC\vh_n, \label{eqn:s4b}
    \end{align}
\end{subequations}
where $\Delta \in \sR$ is a timescale parameter, and $\overline{\mA}, \overline{\mB}$ are discretized counterparts of $\mA, \mB$ via zero-order hold discretization. Specifically, $\overline{\mA} = \exp (\Delta \mA)$, and $\overline{\mB} = (\Delta \mA)^{-1}(\exp (\Delta\mA) - \mI)\cdot \Delta \mB \approx \Delta \mB$. Structured SSMs derive their name from the requirement that the matrix $A$, which governs the temporal dynamics, must adopt a specific structure to enable efficient sequence-to-sequence transformations suitable for deep neural networks. The initial designs introduced were the diagonal plus low-rank (DPLR) structure \cite{gu2022efficiently} and the purely diagonal structure \cite{gu2022parameterization,gupta2022diagonal,smith2023simplified}, with the latter remaining the most widely used.

% \emph{Selective State Space Models}, e.g., \emph{Mamba}~\cite{gu2024mamba}, improves S4 by selectively choosing to focus on or ignore inputs at every timestep. In particular, the parameters $\mB, \mC$, and $\Delta$ are set as the functions of $x_n$, thus becoming input-dependent parameters $\mB_n \mC_n$, and $\Delta_n$, respectively. As a results, the discretized parameters $\overline{\mA}_n = \exp (\Delta_n \mA)$ and $\overline{\mB}_n = \Delta_n \mB_i$ are also input-dependent. \emph{Mamba} chooses $\mB_n = \text{Linear}_{d}(x_n)$, $\mC_n = \text{Linear}_{d}(x_n)$, $\Delta_n = \text{softplus}(\theta + \text{Broadcast}_D(\text{Linear}_1(x_n)))$, where $\text{Linear}_d$ is a parameterized projection to a $d$-dimensional space, $\text{Broadcast}_D$ broadcasts a scalar into a $D$-dimensional vector, and $\theta \in \sR^{D}$ is a learnable parameter vector. 

\emph{Selective State Space Models} (SSMs), such as \emph{Mamba}~\cite{gu2024mamba}, extend S4 by selectively attending to or disregarding inputs at each timestep. Specifically, the parameters $\mB$, $\mC$, and $\Delta$ are defined as functions of the input $x_n$, yielding input-dependent forms $\mB_n$, $\mC_n$, and $\Delta_n$. Consequently, the discretized parameters also become input-dependent, with $\overline{\mA}_n = \exp(\Delta_n \mA)$ and $\overline{\mB}_n = \Delta_n \mB_n$. In \emph{Mamba}, these dependencies are instantiated as  
\begin{align}
\mB_n &= \text{Linear}_{d}(x_n), \nonumber \\
\mC_n &= \text{Linear}_{d}(x_n), \nonumber \\
\Delta_n &= \text{softplus}\!\left(\theta + \text{Broadcast}_D\!\big(\text{Linear}_1(x_n)\big)\right), \nonumber
\end{align} 
where $\text{Linear}_{d}$ denotes a learnable projection into a $d$-dimensional space, $\text{Broadcast}_D$ expands a scalar into a $D$-dimensional vector, and $\theta \in \mathbb{R}^D$ is a learnable parameter vector.

Compared to S4, \emph{Mamba} demonstrates better performance on information-dense data, such as language, particularly as the state dimension $d$ increases, thereby enhancing its information capacity \un{~\cite{li2024mamba, gu2024mamba}} \tmn{Need some citations here to justify the good performance of Mamba}. However, Mamba is still restricted to first-order dynamics, thereby still having difficulty in capture long-range dependencies in long input sequences. Our Proposition~\ref{prop:mamba-limit} proved that Mamba indeed suffers from vanishing and exploding gradient issues. 
\tmn{We need a proposition here.}
\un{\begin{proposition}[Vanishing Gradients in Mamba]
\label{prop:mamba-limit}
Let $\{h_n\}$ be the hidden states of the Mamba architecture defined by
\[
h_n = \overline{A}_n h_{n-1} + \overline{B}_n x_n,
\]
where $\overline{A}_n = \exp(\Delta_n A)$ is diagonal with entries $e^{\Delta_n a_{n,i}}$ for $a_{n,i}<0$ and $\Delta_n>0$. Then the gradient of the loss $L$ with respect to $h_t$ satisfies
\[
\frac{\partial L}{\partial h_t}
= \frac{\partial L}{\partial h_T}\,\prod_{n=t+1}^{T} \overline{A}_n.
\]
If $\min_i a_{n,i}\ll 0$, then
\[
\Big\|\prod_{n=t+1}^{T}\overline{A}_n\Big\|\;\rightarrow 0 
\quad\text{as}\quad T-t\to\infty,
\]
so gradients vanish exponentially with sequence length.
\end{proposition}
\begin{proof}
By the chain rule,
\[
\frac{\partial L}{\partial h_t}
= \frac{\partial L}{\partial h_T}\cdot \frac{\partial h_T}{\partial h_t}.
\]
Unrolling the recurrence yields
\[
\frac{\partial L}{\partial h_t}
= \frac{\partial L}{\partial h_T}\cdot \prod_{n=t+1}^{T}\frac{\partial h_n}{\partial h_{n-1}}
= \frac{\partial L}{\partial h_T}\cdot \prod_{n=t+1}^{T}\overline{A}_n,
\]
since $\partial h_n/\partial h_{n-1} = \overline{A}_n$.  
Now, $\overline{A}_n$ is diagonal with entries $e^{\Delta_n a_{n,i}}$ where $a_{n,i}<0$. Thus,
\[
0 < e^{\Delta_n a_{n,i}} < 1 \quad \forall i,
\]
meaning each factor strictly contracts the corresponding gradient component. Repeated multiplication across $T-t$ steps yields exponential decay in the gradient magnitude. This aligns with the classical description of the \emph{vanishing gradient} \cite{bengio1994learning}, where Jacobians with eigenvalues strictly less than one in modulus drive gradients towards zero as the horizon grows.
\end{proof}}
We further provide empirical evidence to validate Proposition~\ref{prop:mamba-limit} in Figure~\ref{fig:vanishing} below. \tmn{We need an empirical result to show the limitation of Mamba here.}

% Formally, the baseline Mamba recurrence is given by
% \begin{align}
%     h_n = \bar{\boldsymbol{A}}_n h_{n-1} + \bar{\boldsymbol{B}}_n x_n, \label{eq:mamba_update}
% \end{align}
% where $\bar{\boldsymbol{A}}_n = \exp(\Delta_n A)$ and $\bar{\boldsymbol{B}}_n = (\Delta_n A)^{-1}(\bar{\boldsymbol{A}}_n - I)\Delta_n B(x_n)$ are derived from continuous-time parameters. The step size $\Delta_n = \mathrm{softplus}(\mathrm{Linear}(x_n))$, input projection $B(x_n)$, and output projection $C(x_n)$ are input-dependent, while $A$ is a fixed base matrix.
